Observation of the rare baryonic decay $B^{+}\rightarrow p \bar{\it{\Lambda}}$ and measurement of its weak decay parameter

The first observation of the decay $B^{+}\rightarrow p \bar{\it{\Lambda}}$ is presented, using proton-proton collision data collected by the LHCb experiment between 2016 and 2018 at a center-of-mass energy of 13 TeV, corresponding to an integrated luminosity of $5.4\,\mathrm{fb}^{-1}$. The signal significance exceeds seven standard deviations. Using the $B^{+} \rightarrow K^{\mathrm{0}}_{\mathrm{S}} \pi^{+}$ decay as a normalization channel, the branching fraction is measured and combined with previous LHCb results based on data collected at 7 and 8 TeV in 2011 and 2012, yielding $\mathcal{B}(B^{+}\rightarrow p \bar{\it{\Lambda}})=(1.24\pm 0.17\pm 0.05\pm 0.03)\times 10^{-7}$, where the first uncertainty is statistical, the second is systematic, and the third comes from the uncertainty on the branching fraction of the normalization channel. The $B^{+}\rightarrow p \bar{\it{\Lambda}}$ weak decay parameter is measured to be $\alpha_B = 0.87_{-0.29}^{+0.26} \pm 0.09$, indicating the presence of comparable S-wave and P-wave decay amplitudes.

==> Authorship_LHCb-PAPER-2025-044-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
R.  Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
P. Andreola,
M. Andreotti,
S.  Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L.  Arnone,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'{i}de Da Silva,
M. Atzeni,
B. Audurier,
J. A.  Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A.  Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P. B.  Battista,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. A.  Behling,
S. Belin,
A.  Bellavista,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
F. Betti,
J.  Bex,
O. Bezshyyko,
S.  Bhattacharya,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C. Bolognani,
R. Bolzonella,
R. B.  Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E.  Bottalico,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J. D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
J. Brown,
D. Brundu,
E. Buchanan,
M.  Burgos Marcos,
A.T. Burke,
C. Burr,
C.  Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y.  Cai,
A. Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
M.  Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I.  Celestino,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
H.  Chang,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
R.  Cheaib,
M. Chefdeville,
C. Chen,
J.  Chen,
S. Chen,
Z. Chen,
A.  Chen Hu,
M.  Cherif,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S.  Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J.  Connaughton,
A. Contu,
N. Cooke,
G. Cordova,
C.  Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
G. Darze,
A.  Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S.  Dekkers,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
Y.  Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
A.  Doheny,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D.  Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
S.  Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K.   Farmer,
F.  Fassin,
D. Fazzini,
L. Felkowski,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A.  Fomin,
M. Fontana,
L. A.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F{\"u}hring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
P.  Gardner,
L. Garrido,
C. Gaspar,
A.  Gavrikov,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
L.  Golinka-Bezshyyko,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W.  Gomulka,
I. Gonçales Vaz,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.  Haken,
G.  Hallett,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. H.  Harris,
M. Hartmann,
S. Hashmi,
J. He,
N.  Heatley,
A.  Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A.  Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D. C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Iniukhin,
A.  Iohner,
A. Ishteev,
K. Ivshin,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
B.K. Jashal,
A. Jawahery,
C.  Jayaweera,
V. Jevtic,
Z.  Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
E. Jimenez Moya,
N.  Jindal,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
K.  Kalecinska,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
A. Kleimenova,
D. K.  Klekots,
K. Klimaszewski,
M.R. Kmiec,
T.  Knospe,
R.  Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
A.  Korchin,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E.  Kowalczyk,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
O.  Kravcov,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I.  Kyryllin,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. D. Lesser,
B. Leverington,
A. Li,
C.  Li,
C.  Li,
H. Li,
J. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q.  Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Y.  Li,
Z. Lian,
Q.  Liang,
X. Liang,
Z.  Liang,
S. Libralon,
A.  Lightbody,
C. Lin,
T. Lin,
R. Lindner,
H.  Linton,
R. Litvinov,
D. Liu,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
G. Loachamin Ordonez,
I.  Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F. C. L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C.  Lopez Iribarnegaray,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
H.  Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F. M.  Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D.  Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A.  Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
D. Mendoza Granada,
P.  Menendez Valdes Perez,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
R.  Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A.  Moro,
J. Moron,
W.  Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
V.  Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
E.  Nekrasova,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
L.  Nisi,
Q. Niu,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E.  Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L.  Palini,
M. Palutan,
C.  Pan,
X.  Pan,
S. Panebianco,
S. Paniskaki,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D.  Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
X.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
M.  Pereira Martinez,
A. Pereiro Castro,
C.  Perez,
P. Perret,
A.  Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
S.  Pezzulo,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R. N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A.  Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Q.  Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
R.  Racz,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M.  Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F.  Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
S. E. R. Sacha Emile R.,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G.  Scriven,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
B.  Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
W. S.  Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
M.  Singha,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
K. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
K.  Solovieva,
N. S.  Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M.  Stefaniak,
E.N. Stein,
O. Steinkamp,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
J.  Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
P. Svihra,
V. Svintozelskyi,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y. T.  Tang,
M.D. Tat,
J. A. Teijeiro Jimenez,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A. R.  Thomson-Strong,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T. T.  Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
A.  Upadhyay,
B.  Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A.  Vaitkevicius,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.  Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D.  Vico Benet,
P.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
A.  Wang,
B.  Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Y. Wang,
Y. H.  Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z.  Weida,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M. A. Wiegertjes,
C.  Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M. J. Williams,
M.R.J. Williams,
R. Williams,
S.  Williams,
Z.  Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E.  Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T. X.  Xing,
A. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S.  Yadav,
K.  Yang,
X. Yang,
Y. Yang,
Y.  Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
X.  Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
J. A. Zamora Saa,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
R. Zhang,
S. Zhang,
S.~L.~  Zhang,
Y. Zhang,
Y. Z.  Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
Y.  Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica

==> mciteplus.tex <==
%% mciteplus.sty
%% enhanced mcite
%% Version 1.1, 2008/09/30
%%
%% Copyright (c) 2008 Michael Shell
%% Support site:
%% http://www.michaelshell.org/tex/mciteplus/
%%
%%*************************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE! 
%% User assumes all risk.
%% In no event shall any contributor to this code be liable for any damages
%% or losses, including, but not limited to, incidental, consequential, or
%% any other damages, resulting from the use or misuse of any information
%% contained here.
%%
%% All comments are the opinions of their respective authors.
%%
%% This work is distributed under the LaTeX Project Public License (LPPL)
%% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
%% distributed and modified. A copy of the LPPL, version 1.3, is included
%% in the base LaTeX documentation of all distributions of LaTeX released
%% 2003/12/01 or later.
%% Retain all contribution notices and credits.
%% ** Modified files should be clearly indicated as such, including  **
%% ** renaming them and changing author support contact information. **
%%**********************************************************************




\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{mciteplus}[2008/09/30 v1.1 enhanced mcite]

% package option conditionals
\newif\if@OPTIONmcitenohooks\@OPTIONmcitenohooksfalse
\newif\if@OPTIONmcitechapterbibrootbib\@OPTIONmcitechapterbibrootbibfalse
\newif\if@OPTIONmcitedebug\@OPTIONmcitedebugfalse


\DeclareOption{debug}{\global\@OPTIONmcitedebugtrue}
\DeclareOption{nohooks}{\global\@OPTIONmcitenohookstrue}
% use ds@ for chapterbibrootbib to keep option local
\def\ds@chapterbibrootbib{\global\@OPTIONmcitechapterbibrootbibtrue}

\ProcessOptions

% first entry in citation or bibliography flag
\newif\if@mcitefirstentry
% first head entry in citation or bibliography flag
\newif\if@mcitefirstheadentry
% entry using star (is a tail) flag
\newif\if@mcitestarentry
% head declared more than once flag
\newif\if@mciteheadredeclared
% sublist block is open flag
\newif\if@mcitesublistopen
% bst indicates that end punctuation would normally be used
\newif\ifmciteBstWouldAddEndPunct


% flag to indicate that the label widths have changed
% and that LaTeX has to be rerun
\newif\if@mciteLaTeXrerun\@mciteLaTeXrerunfalse

% flag to indicate the use of the first optional argument of a macro
\newif\ifmciteMacroOptArgI\mciteMacroOptArgIfalse
% flag to indicate the use of the first optional argument of a macro (local, non user, use)
\newif\if@mciteLocalMacroOptArgI\@mciteLocalMacroOptArgIfalse
% flag to indicate the use of the second optional argument of a macro
\newif\ifmciteMacroOptArgII\mciteMacroOptArgIIfalse
% flag to indicate the use of the star form of a macro
\newif\ifmciteMacroStarForm\mciteMacroStarFormfalse
% flag to indicate the use of the star form of the \cite forwarding macro
\newif\ifmciteCiteStarFwdArg\mciteCiteStarFwdArgfalse
% flag to indicate the use of the sec ID argument for the \cite forwarding macro
\newif\if@mciteCiteSecIDArg\@mciteCiteSecIDArgfalse

% flag to indicate the use of the first optional argument of a bibitem
\newif\ifmciteBibitemOptArgI\mciteBibitemOptArgIfalse
% flag to indicate the use of the first optional argument of the current head bibitem
\newif\ifmciteCurheadBibitemOptArgI\mciteCurheadBibitemOptArgIfalse


% temporary token list
\newtoks\@mcitetmptoksA
% macro to add (unexpanded) to token list
\def\@mciteAppendToTmpToksA#1{\@mcitetmptoksA=\expandafter{\the\@mcitetmptoksA#1}}


% temporary dimen registers
\newdimen\@mcitetmpdima
\newdimen\@mcitetmpdimb

% temporary count registers
\newcount\@mcitetmpcnta
\newcount\@mcitetmpcntb

% count of entries
\newcounter{mcitebibitemcount}
\setcounter{mcitebibitemcount}{0}
% count of sub items
\newcounter{mcitesubitemcount}


% the default entry punctuation and separator
\providecommand{\mcitedefaultmidpunct}{;\space}
\providecommand{\mcitedefaultendpunct}{.}
\providecommand{\mcitedefaultseppunct}{\relax}
% the default sublist label, begin and end macros
\providecommand{\mcitedefaultsublistlabel}{\alph{mcitesubitemcount})\space}
\providecommand{\mcitedefaultsublistbegin}{\relax}
\providecommand{\mcitedefaultsublistend}{\relax}
% the default max width forms
\providecommand{\mcitedefaultmaxwidthbibitemform}{\arabic{mcitebibitemcount}}
\providecommand{\mcitedefaultmaxwidthbibitemforminit}{\mciteorgbibsamplelabel}
\providecommand{\mcitedefaultmaxwidthsubitemform}{\alph{mcitesubitemcount})}
\providecommand{\mcitedefaultmaxwidthsubitemforminit}{a)}

% sample label which is forwarded to \thebibliography
\def\mcitebibsamplelabel{\rule{\mcitemaxwidthbibitem sp}{0.2pt}}



% Aux and track handles
%
% aux used by \mcite
\def\mciteauxout{\@auxout}
% aux used within \mcitethebibliography
\def\mcitebibauxout{\@mainaux}
% current auxout in use
\def\@mcitecurauxout{\mciteauxout}

% This is the unique ID string used to track multiple bibliographies.
\def\mcitetrackID{main}
% for \mcitethebibliography
\def\mcitebibtrackID{main}
% current Track ID in use
\def\@mcitecurtrackID{\mcitetrackID}


% macros for letter code and string tests
\def\@mciteMacrod{d}
\def\@mciteMacron{n}
\def\@mciteMacros{s}
\def\@mciteMacrob{b}
\def\@mciteMacrof{f}
\def\@mciteMacroh{h}
\def\@mciteMacrobibitem{bibitem}
\def\@mciteMacrosubitem{subitem}



% sets the punctuation bst hooks
\long\def\mciteSetBstMidEndSepPunct#1#2#3{\long\def\mcitebstmidpunct{#1}\relax
                                     \long\def\mcitebstendpunct{#2}\long\def\mcitebstseppunct{#3}}
% sets the actual punctuation used
\long\def\mciteSetMidEndSepPunct#1#2#3{\long\def\mcitemidpunct{#1}\relax
                                  \long\def\mciteendpunct{#2}\long\def\mciteseppunct{#3}}

% sets the sublabel bst hooks
\long\def\mciteSetBstSublistLabelBeginEnd#1#2#3{\long\def\mcitebstsublistlabel{#1}\relax
\long\def\mcitebstsublistbegin{#2}\long\def\mcitebstsublistend{#3}}
% sets the actual sublabel used
\long\def\mciteSetSublistLabelBeginEnd#1#2#3{\long\def\mcitesublistlabel{#1}\relax
\long\def\mcitesublistbegin{#2}\long\def\mcitesublistend{#3}}




% sublist mode flags, b and first forms should be set to false unless \@mcitesublistmode is also true
\newif\if@mcitesublistmode\@mcitesublistmodefalse
\newif\if@mcitesublistmodeb\@mcitesublistmodebfalse
\newif\if@mcitesublistmodef\@mcitesublistmodeffalse
\newif\if@mcitesublistmodeh\@mcitesublistmodehfalse
% reset entry counter flag
\newif\ifmciteResetBibitemCount\mciteResetBibitemCounttrue
% error on unknown entries
\newif\ifmciteErrorOnUnknown\mciteErrorOnUnknowntrue


% BST can request a sublist mode using \mciteSetBstSublistMode, but user requests can override it:
% d = default, use current settings
% n = no sublist
% s = sublist
% b = sublistb
% f = sublistfirst
% h = sublistfirst, including single heads
% note that the changes here are local and will not be remembered outside of the \mcitethebibliography environment
\def\mciteSetBstSublistMode#1{\edef\@mcitetemp{#1}\relax
% only make changes if the user mode allows
\ifx\@mcitesublistmode\@mciteMacrod\relax
  \ifx\@mcitetemp\@mciteMacrod
    \def\@mcitebstsublistmode{d}\else
    \ifx\@mcitetemp\@mciteMacron
      \def\@mcitebstsublistmode{n}\@mcitesublistmodefalse\@mcitesublistmodebfalse\@mcitesublistmodeffalse\@mcitesublistmodehfalse\else
      \ifx\@mcitetemp\@mciteMacros
        \def\@mcitebstsublistmode{s}\@mcitesublistmodetrue\@mcitesublistmodebfalse\@mcitesublistmodeffalse\@mcitesublistmodehfalse\else
        \ifx\@mcitetemp\@mciteMacrob
          \def\@mcitebstsublistmode{b}\@mcitesublistmodetrue\@mcitesublistmodebtrue\@mcitesublistmodeffalse\@mcitesublistmodehfalse\else
          \ifx\@mcitetemp\@mciteMacrof
            \def\@mcitebstsublistmode{f}\@mcitesublistmodetrue\@mcitesublistmodebfalse\@mcitesublistmodeftrue\@mcitesublistmodehfalse\else
            \ifx\@mcitetemp\@mciteMacroh
              \def\@mcitebstsublistmode{h}\@mcitesublistmodetrue\@mcitesublistmodebfalse\@mcitesublistmodeftrue\@mcitesublistmodehtrue\else
              \PackageError{mciteplus}{Unknown mode `#1' in argument to \protect\mciteSetBstSublistMode}%
              {Only `d', `n', `s', `b', `f' and `h' are valid.}\relax
            \fi
          \fi
        \fi
      \fi
    \fi
  \fi
\fi}


% User can specify a sublist mode:
% d = default, use current settings, allow BST to choose
% n = no sublist
% s = sublist
% b = sublistb
% f = sublistfirst
% h = sublistfirst, including single heads
\def\mciteSetSublistMode#1{\edef\@mcitetemp{#1}\relax
\ifx\@mcitetemp\@mciteMacrod
  \def\@mcitesublistmode{d}\else
  \ifx\@mcitetemp\@mciteMacron
    \def\@mcitesublistmode{n}\@mcitesublistmodefalse\@mcitesublistmodebfalse\@mcitesublistmodeffalse\@mcitesublistmodehfalse\else
    \ifx\@mcitetemp\@mciteMacros
      \def\@mcitesublistmode{s}\@mcitesublistmodetrue\@mcitesublistmodebfalse\@mcitesublistmodeffalse\@mcitesublistmodehfalse\else
      \ifx\@mcitetemp\@mciteMacrob
        \def\@mcitesublistmode{b}\@mcitesublistmodetrue\@mcitesublistmodebtrue\@mcitesublistmodeffalse\@mcitesublistmodehfalse\else
        \ifx\@mcitetemp\@mciteMacrof
          \def\@mcitesublistmode{f}\@mcitesublistmodetrue\@mcitesublistmodebfalse\@mcitesublistmodeftrue\@mcitesublistmodehfalse\else
          \ifx\@mcitetemp\@mciteMacroh
            \def\@mcitesublistmode{h}\@mcitesublistmodetrue\@mcitesublistmodebfalse\@mcitesublistmodeftrue\@mcitesublistmodehtrue\else
            \PackageError{mciteplus}{Unknown mode `#1' in argument to \protect\mciteSetSublistMode}%
            {Only `d', `n', `s', `b', `f' and `h' are valid.}\relax
          \fi
        \fi
      \fi
    \fi
  \fi
\fi}




% checks to see if valid type in \@mciteformtypeArg (bibitem or subitem), errors if not
% #1 is name of calling macro
\def\@mcitecheckformtypeerror#1{\relax
\ifx\@mciteformtypeArg\@mciteMacrobibitem\relax
\else
  \ifx\@mciteformtypeArg\@mciteMacrosubitem\relax
  \else
    \PackageError{mciteplus}{Unknown form type  `\@mciteformtypeArg' in argument to \protect#1}%
                            {Only `bibitem' and `subitem' are valid.}\relax
  \fi
\fi}


% sets the bst max width forms
% usage: \mciteSetBstMaxWidthForm[init]{type}{form}
% where type is bibitem or subitem
% if [init] not given, uses \mcitedefaultmaxwidth[TYPE]forminit
\def\mciteSetBstMaxWidthForm{\@ifnextchar[{\@mciteLocalMacroOptArgItrue\@mciteSetBstMaxWidthForm}{\@mciteLocalMacroOptArgIfalse\@mciteSetBstMaxWidthForm[\relax]}}
\def\@mciteSetBstMaxWidthForm[#1]#2#3{\edef\@mciteformtypeArg{#2}\relax
\@mcitecheckformtypeerror{\mciteSetBstMaxWidthForm}\relax
\expandafter\def\csname mcitebstmaxwidth\@mciteformtypeArg form\endcsname{#3}\relax
\if@mciteLocalMacroOptArgI
\expandafter\def\csname mcitebstmaxwidth\@mciteformtypeArg forminit\endcsname{#1}\relax
\else
\expandafter\expandafter\expandafter\def\expandafter\expandafter\csname mcitebstmaxwidth\@mciteformtypeArg forminit\endcsname\expandafter{\csname mcitedefaultmaxwidth\@mciteformtypeArg forminit\endcsname}\relax
\fi}

% sets the max width forms
% usage: \mciteSetMaxWidthForm[init]{type}{form}
% where type is bibitem or subitem
% if [init] not given, uses \mcitebstmaxwidth[TYPE]forminit
\def\mciteSetMaxWidthForm{\@ifnextchar[{\@mciteLocalMacroOptArgItrue\@mciteSetMaxWidthForm}{\@mciteLocalMacroOptArgIfalse\@mciteSetMaxWidthForm[\relax]}}
\def\@mciteSetMaxWidthForm[#1]#2#3{\edef\@mciteformtypeArg{#2}\relax
\@mcitecheckformtypeerror{\mciteSetMaxWidthForm}\relax
\expandafter\def\csname mcitemaxwidth\@mciteformtypeArg form\endcsname{#3}\relax
\if@mciteLocalMacroOptArgI
\expandafter\def\csname mcitemaxwidth\@mciteformtypeArg forminit\endcsname{#1}\relax
\else
\expandafter\expandafter\expandafter\def\expandafter\expandafter\csname mcitemaxwidth\@mciteformtypeArg forminit\endcsname\expandafter{\csname mcitebstmaxwidth\@mciteformtypeArg forminit\endcsname}\relax
\fi}




% initialize punctuation, sublist and maxwidth hooks
%
% punctuation controls
% default is to hook into the bst
\mciteSetMidEndSepPunct{\mcitebstmidpunct}{\mcitebstendpunct}{\mcitebstseppunct}
% the default bst setting is to use the package defaults
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}{\mcitedefaultendpunct}{\mcitedefaultseppunct}
%
% sublist controls
% default sublist mode is to use the defaults
\mciteSetBstSublistMode{d}
\mciteSetSublistMode{d}
% the default sublabel bst setting is to use the package defaults
\mciteSetBstSublistLabelBeginEnd{\mcitedefaultsublistlabel}{\mcitedefaultsublistbegin}{\mcitedefaultsublistend}
% default sublabel setting is to hook into the bst settings
\mciteSetSublistLabelBeginEnd{\mcitebstsublistlabel}{\mcitebstsublistbegin}{\mcitebstsublistend}
%
% max width form controls
% the default max width form bst settings is to use the package defaults
\mciteSetBstMaxWidthForm[\mcitedefaultmaxwidthbibitemforminit]{bibitem}{\mcitedefaultmaxwidthbibitemform}
\mciteSetBstMaxWidthForm[\mcitedefaultmaxwidthsubitemforminit]{subitem}{\mcitedefaultmaxwidthsubitemform}
% the default max width form settings is to hook into the bst settings
\mciteSetMaxWidthForm[\mcitebstmaxwidthbibitemforminit]{bibitem}{\mcitebstmaxwidthbibitemform}
\mciteSetMaxWidthForm[\mcitebstmaxwidthsubitemforminit]{subitem}{\mcitebstmaxwidthsubitemform}




% Defines a macro to track the status of entries. An example showing the
% format is \@mciteEntryStatus@1@Smith98
% where the 1 is the tracking ID, and Smith98 is the cite key.
% Possible values for this status macro are:
% 0 = not yet determined
% 1 = tail   (tail entry following a head entry)
% 2 = head   (head entry followed by one or more tails)
% 3 = single (head entry not followed by any tails)
% usage: \@mciteSetEntryStatus{track ID}{cite key}{status}
\def\@mciteSetEntryStatus#1#2#3{\expandafter\xdef\csname @mciteEntryStatus@#1@#2\endcsname{#3}\relax
%\typeout{SetEntryStatus: Track:`#1' Key:`#2' Status:`#3'}\relax
}
% used to obtain status of a given cite key
% usage: \@mciteGetEntryStatus*{track ID}{cite key}{status out}
% star form: no error checking
\def\@mciteGetEntryStatus{\@ifstar{\@mciteGetEntryStatusStar}{\@mciteGetEntryStatusNoStar}}

\def\@mciteGetEntryStatusStar#1#2#3{\expandafter\let\expandafter#3\csname @mciteEntryStatus@#1@#2\endcsname}

\def\@mciteGetEntryStatusNoStar#1#2#3{\expandafter\let\expandafter#3\csname @mciteEntryStatus@#1@#2\endcsname\relax
\ifx#3\relax
\ifmciteErrorOnUnknown
\PackageError{mciteplus}{Entry Status for cite key `#2' under tracking ID `#1' is undefined, treating it as a head entry}{I don't have a
record of the head/tail status of this citation. Possible reasons include the use
of a cite command that is not mciteplus aware, the use of `\string\nocite{*}', or a problem with the
tracking ID and/or aux file handles. `\string\mciteErrorOnUnknownfalse' can be used to disable this error message.}\relax
\fi
\expandafter\def#3{3}\relax
\fi}


% set head key for given tail
% usage: \@mciteSetHeadofTail{track ID}{tail cite key}{head cite key}
\def\@mciteSetHeadofTail#1#2#3{\expandafter\xdef\csname @mciteHeadofTail@#1@#2\endcsname{#3}}
% get head key for given tail
% usage: \@mciteGetHeadofTail{track ID}{tail cite key}{head key out}
% star form: no error checking
\def\@mciteGetHeadofTail{\@ifstar{\@mciteGetHeadofTailStar}{\@mciteGetHeadofTailNoStar}}

\def\@mciteGetHeadofTailStar#1#2#3{\expandafter\let\expandafter#3\csname @mciteHeadofTail@#1@#2\endcsname}

\def\@mciteGetHeadofTailNoStar#1#2#3{\expandafter\let\expandafter#3\csname @mciteHeadofTail@#1@#2\endcsname\relax
\ifx#3\relax
\PackageError{mciteplus}{Head for tail cite key `#2' under tracking ID `#1' is undefined}{I don't have a
record of the head key of this citation.}\relax
\fi}


% for debug status messages
% converts given status number to word description
\def\@mciteStatusNumToWord#1{\expandafter\ifcase#1\relax
Unknown\or Tail\or Head with tails\or Head without tails\else Invalid (#1)\fi}
% form that makes no distinction between status 2 or 3. Used with \cite debug as 
% head status is not finalized till after the entry group
\def\@mciteStatusNumToWordH#1{\expandafter\ifcase#1\relax
Unknown\or Tail\or Head\or Head\else Invalid (#1)\fi}




% usage:\mciteSetMaxWidth{track ID}{type}{width}
% Defines a macro to track the max width of a given label type.
% An example showing the format is \@mciteMaxWidthStore@main@bibitem
% which is set globally
% we don't use @ in the macro name as this cmd appears in the aux
\def\mciteSetMaxWidth#1#2#3{\edef\@mciteformtypeArg{#2}\relax
\@mcitecheckformtypeerror{\mciteSetMaxWidth}\relax
\expandafter\xdef\csname @mciteMaxWidthStore@#1@\@mciteformtypeArg\endcsname{#3}}
%
% usage:\mciteGetMaxWidth{track ID}{type}{out macro}
% reads the stored max width of the given label type into the out macro
% which is set globally
\def\mciteGetMaxWidth#1#2#3{\edef\@mciteformtypeArg{#2}\relax
\@mcitecheckformtypeerror{\mciteGetMaxWidth}\relax
\expandafter\global\expandafter\let\expandafter#3\csname @mciteMaxWidthStore@#1@\@mciteformtypeArg\endcsname}

% usage:\mciteSetMaxCount{track ID}{type}{count}
% Defines a macro to track the max count of a given label type.
% An example showing the format is \@mciteMaxCountStore@main@bibitem
% which is set globally
% we don't use @ in the macro name as this cmd appears in the aux
\def\mciteSetMaxCount#1#2#3{\edef\@mciteformtypeArg{#2}\relax
\@mcitecheckformtypeerror{\mciteSetMaxCount}\relax
\expandafter\xdef\csname @mciteMaxCountStore@#1@\@mciteformtypeArg\endcsname{#3}}
%
% usage:\mciteGetMaxCount{track ID}{type}{out macro}
% reads the stored max count of the given label type into the out macro
% which is set globally
\def\mciteGetMaxCount#1#2#3{\edef\@mciteformtypeArg{#2}\relax
\@mcitecheckformtypeerror{\mciteGetMaxCount}\relax
\expandafter\global\expandafter\let\expandafter#3\csname @mciteMaxCountStore@#1@\@mciteformtypeArg\endcsname}


% sets \mcitemaxcountbibitem and \mcitemaxcountsubitem via \mciteGetMaxCount globally
% sets them to zero if \mciteGetMaxCount returns \relax
% clears \@mcitecorrectmaxcountbibitem and \@mcitecorrectmaxcountsubitem
% uses \@mcitecurtrackID
\def\@mciteMaxCountInitialize{\mciteGetMaxCount{\@mcitecurtrackID}{bibitem}{\mcitemaxcountbibitem}\relax
\ifx\mcitemaxcountbibitem\relax\gdef\mcitemaxcountbibitem{0}\fi
\mciteGetMaxCount{\@mcitecurtrackID}{subitem}{\mcitemaxcountsubitem}\relax
\ifx\mcitemaxcountsubitem\relax\gdef\mcitemaxcountsubitem{0}\fi
\global\let\mcitemaxcountbibitem\mcitemaxcountbibitem
\global\let\mcitemaxcountsubitem\mcitemaxcountsubitem
\xdef\@mcitecorrectmaxcountbibitem{0}\relax
\xdef\@mcitecorrectmaxcountsubitem{0}\relax}
%
% usage: \@mciteMaxCountUpdate
% updates \@mcitecorrectmaxcountsubitem
% no need for \@mcitecorrectmaxcountbibitem as this is carried by the counter itself
\def\@mciteMaxCountUpdate{\relax
\ifnum\@mcitecorrectmaxcountsubitem<\arabic{mcitesubitemcount}\relax
  \xdef\@mcitecorrectmaxcountsubitem{\arabic{mcitesubitemcount}}\relax
\fi}
%
% usage: \@mciteMaxCountAuxWrite uses \@mcitecurauxout and \@mcitecurtrackID
% writes \mciteSetMaxCount{track ID}{type}{count} to \@mcitecurauxout
% and warns if correct values do not match \mcitemaxcountbibitem, \mcitemaxcountsubitem
\def\@mciteMaxCountAuxWrite{\relax
\if@filesw
  \immediate\write\@mcitecurauxout{\string\mciteSetMaxCount{\@mcitecurtrackID}{bibitem}{\arabic{mcitebibitemcount}}}\relax
  \immediate\write\@mcitecurauxout{\string\mciteSetMaxCount{\@mcitecurtrackID}{subitem}{\@mcitecorrectmaxcountsubitem}}\relax
\fi
\ifnum\mcitemaxcountbibitem=\arabic{mcitebibitemcount}\relax
  \ifnum\mcitemaxcountsubitem=\@mcitecorrectmaxcountsubitem\relax\else
    \@latex@warning@no@line{Mciteplus max count has changed}\global\@mciteLaTeXreruntrue
  \fi
\else
  \@latex@warning@no@line{Mciteplus max count has changed}\global\@mciteLaTeXreruntrue
\fi}


% usage: \@mciteMaxWidthInitialize{type}
% sets \mcitemaxwidth[TYPE] via \GetMaxWidth globally
% if \GetMaxWidth returns \relax, sets them to the width (without sp units at end) of \mcitebstmaxwidth[TYPE]forminit
% as evaluated when bibitem and subitem counters are both = 1
% clears \@mcitecorrectmaxwidth[TYPE] globally to 0
% uses \@mcitecurtrackID
\def\@mciteMaxWidthInitialize#1{\edef\@mcitemaxwidthinitializetypeArg{#1}\relax
\expandafter\mciteGetMaxWidth\expandafter{\expandafter\@mcitecurtrackID\expandafter}\expandafter{\expandafter\@mcitemaxwidthinitializetypeArg\expandafter}\expandafter{\csname mcitemaxwidth#1\endcsname}\relax
\expandafter\ifx\csname mcitemaxwidth#1\endcsname\relax
  \begingroup
  % set counters to 1 locally
  \csname c@mcitebibitemcount\endcsname 1\relax
  \csname c@mcitesubitemcount\endcsname 1\relax
  \settowidth{\@mcitetmpdima}{\csname mcitemaxwidth#1forminit\endcsname}\relax
  \@mcitetmpcnta=\@mcitetmpdima\relax
  \expandafter\xdef\csname mcitemaxwidth#1\endcsname{\the\@mcitetmpcnta}\relax
  \endgroup
\fi
\expandafter\xdef\csname @mcitecorrectmaxwidth#1\endcsname{0}}
%
% usage: \@mciteMaxWidthUpdate{type}
% globally updates \@mcitecorrectmaxwidth[TYPE] based on \mcitemaxwidth[TYPE]form
\def\@mciteMaxWidthUpdate#1{\relax
\settowidth{\@mcitetmpdima}{\csname mcitemaxwidth#1form\endcsname}\relax
\@mcitetmpcnta=\@mcitetmpdima\relax
\@mcitetmpcntb=\csname @mcitecorrectmaxwidth#1\endcsname\relax
\ifnum\@mcitetmpcnta>\@mcitetmpcntb\relax
  \expandafter\xdef\csname @mcitecorrectmaxwidth#1\endcsname{\the\@mcitetmpcnta}\relax
\fi}
%
%
% usage: \@mciteMaxWidthAuxWrite uses \@mcitecurauxout and \@mcitecurtrackID
% writes \mciteSetMaxWidth{track ID}{type}{correct width in sp}
% for both bibitem and subitem to \@mcitecurauxout
% and warns if correct values do not match \mcitemaxwidthbibitem, \mcitemaxwidthsubitem
\def\@mciteMaxWidthAuxWrite{\relax
\if@filesw
  \immediate\write\@mcitecurauxout{\string\mciteSetMaxWidth{\@mcitecurtrackID}{bibitem}{\@mcitecorrectmaxwidthbibitem}}\relax
  \immediate\write\@mcitecurauxout{\string\mciteSetMaxWidth{\@mcitecurtrackID}{subitem}{\@mcitecorrectmaxwidthsubitem}}\relax
\fi
\ifnum\mcitemaxwidthbibitem=\@mcitecorrectmaxwidthbibitem\relax
  \ifnum\mcitemaxwidthsubitem=\@mcitecorrectmaxwidthsubitem\relax\else
    \@latex@warning@no@line{Mciteplus max width has changed}\global\@mciteLaTeXreruntrue
  \fi
\else
  \@latex@warning@no@line{Mciteplus max width has changed}\global\@mciteLaTeXreruntrue
\fi}





% empty \mciteheadlist in case someone trys to access it before a \cite
\def\mciteheadlist{}

% default wrappers for \cite and \nocite, package hooks (e.g., multibbl) can change these later
\def\@mciteCiteWrapper{\mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\mciteOrgcite}}
\def\@mciteNociteWrapper{\mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\mciteOrgnocite}}


% \mcite was undocumented in mcite.sty. We don't need it and it will not work with
% some multibibliography packages. So, we'll not use them.
% mcite version of \cite
%\def\mcite{\mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\mciteOrgcite}}
% mcite version of \nocite
%\def\mnocite{\mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\mciteOrgnocite}}


% mciteplus \cite wrappers
% usage: \mciteCiteA*{aux out}{track ID}{prehandler}{posthandler}{fwd macro}*[opt1][opt2]{cite list}
%        \mciteCiteB*{aux out}{track ID}{prehandler}{posthandler}{fwd macro}*[opt1][opt2]{sec ID}{cite list}
% B form is for \cite that use two arguments, such as that of multibbl.sty
% processes cite list and fowards arguments and list of heads to specified \cite macro
% star form means no default \mciteDoList processing
\DeclareRobustCommand{\mciteCiteA}{\@mciteCiteSecIDArgfalse\@mciteCiteAB}
\DeclareRobustCommand{\mciteCiteB}{\@mciteCiteSecIDArgtrue\@mciteCiteAB}


\def\@mciteCiteAB{\@ifstar{\mciteMacroStarFormtrue\@@mciteCiteAB}{\mciteMacroStarFormfalse\@@mciteCiteAB}}

\def\@@mciteCiteAB#1#2#3#4#5{\def\mciteCiteAuxArg{#1}\def\mciteCiteTrackArg{#2}\def\mciteCitePrehandlerArg{#3}\relax
                             \def\mciteCitePosthandlerArg{#4}\relax\def\mciteCiteFwdArg{#5}\relax
                             \@ifstar{\mciteCiteStarFwdArgtrue\@@@mciteCiteAB}{\mciteCiteStarFwdArgfalse\@@@mciteCiteAB}}

\def\@@@mciteCiteAB{\@ifnextchar[{\mciteMacroOptArgItrue\@@@@mciteCiteAB}%
{\mciteMacroOptArgIfalse\@@@@mciteCiteAB[\relax]}}

\def\@@@@mciteCiteAB[#1]{\def\mciteCiteOptArgI{#1}\relax
\@ifnextchar[{\mciteMacroOptArgIItrue\@@@@@mciteCiteAB}%
{\mciteMacroOptArgIIfalse\@@@@@mciteCiteAB[\relax]}}

\def\@@@@@mciteCiteAB[#1]{\def\mciteCiteOptArgII{#1}\relax
\if@mciteCiteSecIDArg
\def\@mciteNextMacroChain{\@@@@@mciteCiteB}\relax
\else
\let\mciteCiteSecIDArg\relax
\def\@mciteNextMacroChain{\@@@@@@mciteCiteAB}\relax
\fi
\@mciteNextMacroChain}


\def\@@@@@mciteCiteB#1{\def\mciteCiteSecIDArg{#1}\@@@@@@mciteCiteAB}

\def\@@@@@@mciteCiteAB#1{\def\mciteCiteListArg{#1}\relax
\edef\mciteFwdCiteListArg{}\relax
% execute the user's pre-handler code
\mciteCitePrehandlerArg\relax
\ifmciteMacroStarForm
% star form means no mcite default processing
% the user will have to do all of this in their handler
\else
% otherwise, process the cite list and set the forward cite list to the list of heads
\mciteDoList{\mciteCiteAuxArg}{\mciteCiteTrackArg}{\mciteCiteListArg}\relax
\edef\mciteFwdCiteListArg{\mciteheadlist}\relax
% optional additional calls to do lists for duplicate/global bibliographies
\mciteExtraDoLists\relax
\fi
\relax
% execute the user's post-handler code
\mciteCitePosthandlerArg\relax
% build the forwarding macro and arguments list
\@mcitetmptoksA=\expandafter{\mciteCiteFwdArg}\relax
\ifmciteCiteStarFwdArg
\@mciteAppendToTmpToksA{*}\relax
\fi
\ifmciteMacroOptArgI
\@mciteAppendToTmpToksA{[}\relax
\expandafter\@mciteAppendToTmpToksA\expandafter{\mciteCiteOptArgI}\relax
\@mciteAppendToTmpToksA{]}\relax
\fi
\ifmciteMacroOptArgII
\@mciteAppendToTmpToksA{[}\relax
\expandafter\@mciteAppendToTmpToksA\expandafter{\mciteCiteOptArgII}\relax
\@mciteAppendToTmpToksA{]}\relax
\fi
\if@mciteCiteSecIDArg
\expandafter\@mciteAppendToTmpToksA\expandafter{\expandafter{\mciteCiteSecIDArg}}\relax
\fi
\expandafter\@mciteAppendToTmpToksA\expandafter{\expandafter{\mciteFwdCiteListArg}}\relax
\edef\@mciteCiteFwd{\the\@mcitetmptoksA}\relax
% forward to the "real" \cite
\@mciteCiteFwd}


% mciteplus engine
% processes cite list, records status of keys and writes tail (and head)
% citations to aux file
% list of heads is output to \mciteheadlist for forwarding to \cite
% usage: \mciteDoList{aux out}{track ID}{cite list}
% use noauxwrite for aux out to disable writes to aux
\def\mciteDoList#1#2#3{\edef\@mcitecurauxout{#1}\edef\@mcitecurtrackID{#2}\edef\@mcitetemp{#3}\relax
\expandafter\@mciteDoList\expandafter{\@mcitetemp}}

% flag to determine if mciteDoList should write to aux file
\newif\if@mciteDoListwriteaux \@mciteDoListwriteauxtrue
\def\@mciteMacronoauxwrite{noauxwrite}

\def\@mciteDoList#1{\let\@mcitecurhead\relax % reset current head
\@mciteDoListwriteauxtrue
% disable aux writes if aux parameter is "noauxwrite"
\ifx\@mcitecurauxout\@mciteMacronoauxwrite\@mciteDoListwriteauxfalse\fi
\@mcitefirstentrytrue\@mcitefirstheadentrytrue
\def\mciteheadlist{}\def\@mcitecurstatus{\relax}\relax
\@for\@mcitecurkey:=#1\do{\expandafter\@mciteCheckKey\@mcitecurkey\end\relax
% ignore empty keys
\ifx\@mcitecurkey\@empty
% warn about \nocite{*}
\if@mcitestarentry
  \typeout{** WARNING: mciteplus: Wildcard `*' citation entry declared. BibTeX will add untracked entries to the bibliography.}\relax
  % add * to the head list
  \if@mcitefirstentry
    \@mcitefirstentryfalse
    \edef\mciteheadlist{*}\relax
  \else
    \edef\mciteheadlist{\mciteheadlist,*}\relax
  \fi
\fi
\else % key is not empty
% get entry status
\@mciteGetEntryStatus*{\@mcitecurtrackID}{\@mcitecurkey}{\@mcitecurstatus}\relax
% if entry status is undefined, set status number code to undetermined and update \@mcitecurstatus
\ifx\@mcitecurstatus\relax
  \@mciteSetEntryStatus{\@mcitecurtrackID}{\@mcitecurkey}{0}\relax
  \@mciteGetEntryStatus{\@mcitecurtrackID}{\@mcitecurkey}{\@mcitecurstatus}\relax
\fi
\if@mcitestarentry % if declared to be a tail
  \if@mcitefirstheadentry % tail cannot be declared until after a head
    \PackageError{mciteplus}{Tail `\@mcitecurkey' is declared without a valid head}{You have to
                             declare a head citation before entering tail citations in cite list.}\relax
  \fi
  \ifnum\@mcitecurstatus>1\relax % cannot have been previously declared as a head
    \PackageError{mciteplus}{Tail citation `\@mcitecurkey' has previously been declared as a head}{Declare
                             each citation entry as a head or a tail, but not both.}\relax
  \fi
  \if@mciteheadredeclared % the current head has been redeclared, OK with some restrictions
    \ifnum\@mcitecurstatus=0\relax % cannot add new tails to previous group definitions
    \PackageError{mciteplus}{New tail citation `\@mcitecurkey' cannot be added to the already existing
                             definition of group of head `\@mcitecurhead'}{You cannot define a group,
                             then reissue the head and add new tail citations.}\relax
    \fi
    \ifnum\@mcitecurstatus=1\relax % OK to respecify tails as long as they already belong to this group, 
                                   % this allows for overall (global) bibliographies
      \@mciteGetHeadofTail{\@mcitecurtrackID}{\@mcitecurkey}{\@mciteheadofcurkey}\relax
      \ifx\@mciteheadofcurkey\@mcitecurhead
      % Note: We don't/can't catch the case of repeated tail declarations under a redeclared head.
      % Not a mandatory error anyway.
      \else
        % tail cannot have been declared in definition of another group
        \PackageError{mciteplus}{Tail citation `\@mcitecurkey' is not allowed in group of head
                                 `\@mcitecurhead' as this tail has already been declared in group
                                 of head `\@mciteheadofcurkey'}{You cannot have a tail citation
                                 that appears in more than one citation group.}\relax
      \fi
    \fi
  \else % head not redeclared
    \ifnum\@mcitecurstatus=1\relax % the current head has not been declared before, so neither should any of its tails
      \@mciteGetHeadofTail{\@mcitecurtrackID}{\@mcitecurkey}{\@mciteheadofcurkey}\relax
      \ifx\@mciteheadofcurkey\@mcitecurhead
        % tail cannot be declared twice in initial definition, this is an optional error
        \PackageError{mciteplus}{Tail citation `\@mcitecurkey' has been declared more than once in
                                 definition of group for head `\@mcitecurhead'}{Each tail
                                 citation can only be specified once in the definition
                                 of a group.}\relax
      \else
        % tail cannot have been declared in definition of another group
        \PackageError{mciteplus}{Tail citation `\@mcitecurkey' is not allowed in group of head
                                 `\@mcitecurhead' as this tail has already been declared in group
                                 of head `\@mciteheadofcurkey'}{You cannot have a tail citation
                                 that appears in more than one citation group.}\relax
      \fi
    \fi
  \fi% end if head redeclared
  % if not declared before, process as a valid tail
  \ifnum\@mcitecurstatus=0\relax
    % record type as tail
    \@mciteSetEntryStatus{\@mcitecurtrackID}{\@mcitecurkey}{1}\relax
    \@mciteGetEntryStatus{\@mcitecurtrackID}{\@mcitecurkey}{\@mcitecurstatus}\relax
    % write out tail citation to aux as it will not be forwarded to \cite
    \if@mciteDoListwriteaux
      \@mcitewritecurkeytoaux
    \fi
    % record head for this tail
    \@mciteSetHeadofTail{\@mcitecurtrackID}{\@mcitecurkey}{\@mcitecurhead}\relax
    % change current head from code 3 (single) to 2 (one or more tails)
    \@mciteSetEntryStatus{\@mcitecurtrackID}{\@mcitecurhead}{2}\relax
  \fi
\else % is declared to be a head
  \edef\@mcitecurhead{\@mcitecurkey}\relax % this is our new current head
  % add to the head list
  \if@mcitefirstentry
    \@mcitefirstentryfalse
    \edef\mciteheadlist{\@mcitecurkey}\relax
  \else
    \edef\mciteheadlist{\mciteheadlist,\@mcitecurkey}\relax
  \fi
  \@mcitefirstheadentryfalse
  \ifnum\@mcitecurstatus=1\relax % cannot have previously been used as a tail
    \@mciteGetHeadofTail{\@mcitecurtrackID}{\@mcitecurkey}{\@mciteheadofcurkey}\relax
    \PackageError{mciteplus}{Head citation `\@mcitecurkey' has previously been declared
                             as a tail of `\@mciteheadofcurkey'}{Declare each citation
                             entry as a head or a tail, but not both.}\relax
  \fi
  \@mciteheadredeclaredfalse % assume not redeclared
  \ifnum\@mcitecurstatus>1\relax % has already been declared?
    \@mciteheadredeclaredtrue % OK, but do not allow any new future tails for this head
  \fi
  % if not declared before, set as a head, single. Will later change to code 2 if tails are found.
  \if@mciteheadredeclared\else
    \@mciteSetEntryStatus{\@mcitecurtrackID}{\@mcitecurkey}{3}\relax
    \@mciteGetEntryStatus{\@mcitecurtrackID}{\@mcitecurkey}{\@mcitecurstatus}\relax
    % write out head citation to aux.
    % This will result in the entry appearing twice in the aux file as the
    % entry will be part of the \mciteheadlist which will be forwarded to \cite.
    % However, we need to write this out now to preserve the order of the citations.
    \if@mciteDoListwriteaux
      \@mcitewritecurkeytoaux
    \fi
    % this is the new current head
    \let\@mcitecurhead\@mcitecurkey
  \fi % fi not headredeclared
\fi % fi tail or head
% debug report
\if@OPTIONmcitedebug
  \ifnum\@mcitecurstatus=1\relax
  \edef\@mcitedebugheadoftail{Head of this tail: `\@mcitecurhead'}\relax
    \else
  \edef\@mcitedebugheadoftail{}\relax
  \fi
  \typeout{** Mciteplus Debug: Citation Entry: `\@mcitecurkey' TrackID: `\@mcitecurtrackID'
  Auxout: \ifx\@mcitecurauxout\@mciteMacronoauxwrite `none (\@mciteMacronoauxwrite)' \else `\the\@mcitecurauxout' \fi
  Status: `\@mciteStatusNumToWordH{\@mcitecurstatus}' \@mcitedebugheadoftail}\relax
\fi
% end debug report
\fi % only nonempty
}% end do loop
}

% hook to allow for a redo. Useful for global bibliographies
\def\mciteExtraDoLists{\relax}

% determines if an entry starts with an *, removes the * from the start of the entry name
% and sets \@mcitestarentry and \@mcitecurkey accordingly
\def\@mciteCheckKey#1#2\end{\@mcitestarentryfalse
\ifx*#1\@mcitestarentrytrue\edef\@mcitecurkey{#2}\relax
\else
\edef\@mcitecurkey{#1#2}%
\fi}

% writes current key citation to aux. We put this in a macro because some packages
% may fiddle with \if@filesw (making it a macro rather than an if), tripping up
% TeX's parser if \if@filesw is ever within another conditional as is the case
% within \@mciteDoList
\def\@mcitewritecurkeytoaux{\if@filesw\immediate\write\@mcitecurauxout{\string\citation{\@mcitecurkey}}\fi}



% custom \ref command displays \mcitesubrefform when
% \ref'd
% prefix to reference labels to avoid namespace clash
\def\@mcitereflabelprefix{MciteSubReferenceLabel}
\def\@mciteSetSubRefLabel{\begingroup\def\@currentlabel{\mcitesubrefform}\label{\@mcitereflabelprefix:\@mcitecurtrackID:\mciteBibitemArgI}\endgroup}
% default to using the actual sublist form.
\providecommand{\mcitesubrefform}{\arabic{mcitebibitemcount}.\alph{mcitesubitemcount}}
% give user access to sublist \ref and \pageref
% usage: \mciteSubRef[track ID]{cite key}
\def\mciteSubRef{\@ifnextchar[{\@mciteSubRef}{\@mciteSubRef[\mcitetrackID]}}
\def\@mciteSubRef[#1]#2{\ref{\@mcitereflabelprefix:#1:#2}}
\def\mciteSubPageRef{\@ifnextchar[{\@mciteSubPageRef}{\@mciteSubPageRef[\mcitetrackID]}}
\def\@mciteSubPageRef[#1]#2{\pageref{\@mcitereflabelprefix:#1:#2}}


% for debug, head of tail lookup
\def\@mcitecurheadlookup{}




% mciteplus version of \bibitem
% support the optional arg of \bibitem[]{} as well
\def\mcitebibitem{\@ifnextchar[{\global\mciteBibitemOptArgItrue\@mcitebibitem}%
{\global\mciteBibitemOptArgIfalse\@mcitebibitem[\relax]}}

\def\@mcitebibitem[#1]#2{\relax
% build the forwarding macro: \mciteOrgbibitem{#2} or \mciteOrgbibitem[#1]{#2}
\gdef\mciteBibitemOptArgI{#1}\gdef\mciteBibitemArgI{#2}\relax
\@mcitetmptoksA={\mciteOrgbibitem}\relax
\ifmciteBibitemOptArgI
\@mciteAppendToTmpToksA{[}\relax
\expandafter\@mciteAppendToTmpToksA\expandafter{\mciteBibitemOptArgI}\relax
\@mciteAppendToTmpToksA{]}\relax
\fi
\expandafter\@mciteAppendToTmpToksA\expandafter{\expandafter{\mciteBibitemArgI}}\relax
% build the command. we need a global def here so that the changes will persist in spite
% of a later closed sublist
\xdef\@mciteBibitemFwdMacroArgs{\the\@mcitetmptoksA}\relax
% on the very first \bibitem initialize the maxwidths
% we do this here so that the bibstyle can have its say on the forminit
\if@mcitefirstentry
  \@mciteMaxWidthInitialize{bibitem}\relax
  \@mciteMaxWidthInitialize{subitem}\relax
\fi
% get status of entry and process accordingly
\@mciteGetEntryStatus{\@mcitecurtrackID}{#2}{\@mcitecurstatus}\relax
% status get may happen inside a list, so make the changes to \@mcitecurstatus global
\global\let\@mcitecurstatus\@mcitecurstatus
% debug report
\if@OPTIONmcitedebug
  \ifnum\@mcitecurstatus=1\relax
    \@mciteGetHeadofTail{\@mcitecurtrackID}{\mciteBibitemArgI}{\@mcitecurheadlookup}\relax
    \edef\@mcitedebugheadoftail{Head of this tail: `\@mcitecurheadlookup' (from citation),  `\@mcitecurhead' (in bibliography)}\relax
  \else
    \edef\@mcitedebugheadoftail{}\relax
  \fi
  \typeout{** Mciteplus Debug: \string\mcitebibitem\space Entry: `\mciteBibitemArgI' TrackID: `\@mcitecurtrackID'
  Status: `\@mciteStatusNumToWord{\@mcitecurstatus}' \@mcitedebugheadoftail}\relax
\fi
% end debug report
\ifnum\@mcitecurstatus=1\relax % if a tail
  % error if a tail starts the bibliography
  \if@mcitefirstentry
  \PackageError{mciteplus}{Bibliography begins with a tail entry `\mciteBibitemArgI'}{For sorting
                           bibstyles, you must set the `mcitetail' BibTeX database field
                           for each tail entry and use a bibstyle that understands that field.}\relax
  \fi
  \mcitemidpunct\relax
  % open sublist if needed
  \if@mcitesublistmode
    \if@mcitesublistopen\else
      \global\@mcitesublistopentrue
      \relax\mcitesublistbegin\relax
    \fi
    \relax\mcitesublistlabel\relax\@mciteSetSubRefLabel\relax\@mciteMaxWidthUpdate{subitem}\relax
  \fi
  \@mciteMaxCountUpdate
  \addtocounter{mcitesubitemcount}{1}\relax
\else% is head
   \if@mcitefirstentry\else\mciteendpunct\relax\mciteEndOfBibGroupPresubcloseHook\relax\fi
   % close sublist if open
   % watch out with variables as this will close off local changes
   % addtocounter and setcounter make global changes
   \if@mcitesublistopen
     \mcitesublistend\relax
     \global\@mcitesublistopenfalse
   \fi
   \relax\mciteEndOfBibGroupPostsubcloseHook\relax
   % record current head key and argument info
   \xdef\@mcitecurhead{#2}\relax
   \gdef\mciteCurheadBibitemArgI{#2}\relax
   \gdef\mciteCurheadBibitemOptArgI{#1}\relax
   \ifmciteBibitemOptArgI\global\mciteCurheadBibitemOptArgItrue\else\global\mciteCurheadBibitemOptArgIfalse\fi
   % note: with \mcitebibitem mcitebibitemcount advances with heads
   % and holds the current head count until the next \mcitebibitem
   % However, at the end of the \mcitebibitem, mcitesubitemcount
   % is one more than the number of subitems as the label is
   % rendered before updating the counter.
   \setcounter{mcitesubitemcount}{1}\relax
   \addtocounter{mcitebibitemcount}{1}\relax
   \@mciteMaxCountUpdate
   \if@mcitefirstentry\else\relax\mciteseppunct\relax\fi
   \@mciteBibitemFwdMacroArgs\relax\relax\relax
   % check and update the bibitem label width
   \@mciteMaxWidthUpdate{bibitem}\relax
   \ifnum\@mcitecurstatus=2\relax % if head with tails
     \if@mcitesublistmodef
       % open sublist if needed
       \if@mcitesublistopen\else
         \global\@mcitesublistopentrue
         \mcitesublistbegin\relax
       \fi
       \relax\mcitesublistlabel\relax\@mciteSetSubRefLabel\relax\@mciteMaxWidthUpdate{subitem}\relax
       \addtocounter{mcitesubitemcount}{1}\relax
     \fi
   \fi
   \ifnum\@mcitecurstatus=3\relax % if head without tails
     \if@mcitesublistmodeh
       % open sublist if needed
       \if@mcitesublistopen\else
         \global\@mcitesublistopentrue
         \mcitesublistbegin\relax
       \fi
       \relax\mcitesublistlabel\relax\@mciteSetSubRefLabel\relax\@mciteMaxWidthUpdate{subitem}\relax
       \addtocounter{mcitesubitemcount}{1}\relax
     \fi
   \fi
   \if@mcitesublistmodeb
     \addtocounter{mcitesubitemcount}{1}\relax
   \fi
\fi% if tail or head
\global\@mcitefirstentryfalse\ignorespaces}

% End of \bibitem marker from bibstyle
\def\EndOfBibitem{\relax}

% hook inserted at the end of bibitem group, before the sublist is closed
\def\mciteEndOfBibGroupPresubcloseHook{\relax}
% hook inserted at the end of bibitem group, after the sublist is closed
\def\mciteEndOfBibGroupPostsubcloseHook{\relax}

% hook inserted at \mcitethebibliography
\def\mcitethebibliographyHook{\relax}


% hook to allow insertion of custom code at end of mcitethebibliography
\def\mciteBIBdecl{\relax}
% hook to allow insertion of custom code at end of endmcitethebibliography
\def\mciteBIBenddecl{\relax}
% hook to allow insertion of custom code at end of thebibliography
\def\mcitefwdBIBdecl{\relax}




% Bibdecl for package hooks
\def\@mcitepkgBIBdecl{\relax}
% single use internal BIB hook, is automatically reset to \relax at end of \mcitethebibliography
\let\@mciteoneshotBIBdecl\relax


% mciteplus version of \thebibliography
\def\mcitethebibliography#1{\@mcitefirstentrytrue
  \@mcitesublistopenfalse
  \let\@mcitecurauxout\mcitebibauxout
  \let\@mcitecurtrackID\mcitebibtrackID
  \ifmciteResetBibitemCount\setcounter{mcitebibitemcount}{0}\fi
  \setcounter{mcitesubitemcount}{0}\relax
  \xdef\mciteorgbibsamplelabel{#1}\relax
  % set these to something so that init forms that reference them won't choke
  \gdef\mciteBibitemOptArgI{\relax}\relax
  \gdef\mciteBibitemArgI{\relax}\relax
  \global\mciteBibitemOptArgIfalse
  \gdef\mciteCurheadBibitemOptArgI{\relax}\relax
  \gdef\mciteCurheadBibitemArgI{\relax}\relax
  \global\mciteCurheadBibitemOptArgIfalse
  % note: pkg and user hooks may update tracking ID
  \relax\@mcitepkgBIBdecl\relax
  \relax\@mciteoneshotBIBdecl\relax
  \relax\mciteBIBdecl\relax
  \@mciteMaxCountInitialize
  % we initialize here to get a valid \mcitemaxwidthbibitem for \mcitebibsamplelabel
  % but we will reinitialize again at the first \bibitem so that any BST changes can take affect
  \@mciteMaxWidthInitialize{bibitem}\relax
  % debug report
  \if@OPTIONmcitedebug
  \typeout{}\typeout{}\relax
  \typeout{** Mciteplus Debug: \string\mcitethebibliography\space TrackID: `\@mcitecurtrackID' Auxout: `\the\@mcitecurauxout'}\relax
  \fi
  % end debug report
  \thebibliography{\mcitebibsamplelabel}\relax
  \mcitethebibliographyHook\relax
  \relax\mcitefwdBIBdecl\relax
  \let\mciteOrgbibitem\bibitem
  \def\bibitem{\mcitebibitem}}

\def\endmcitethebibliography{\mciteendpunct\relax
  \relax\mciteEndOfBibGroupPresubcloseHook\relax
  % close sublist if open
  \if@mcitesublistopen
    \mcitesublistend\relax
    \@mcitesublistopenfalse
  \fi
  \relax\mciteEndOfBibGroupPostsubcloseHook\relax
  \relax\mciteBIBenddecl\relax
  % globally clear oneshot decl
  \global\let\@mciteoneshotBIBdecl\relax
  % restore original \bibitem as some \endthebibliography tack notes at the end (e.g., REVTeX)
  % we'll add them to the count with mcite's counters and continue to track the bibitem width
  \setcounter{mcitesubitemcount}{1}\relax
  \def\bibitem{\addtocounter{mcitebibitemcount}{1}\@mciteMaxWidthUpdate{bibitem}\relax\mciteOrgbibitem}
  \endthebibliography\relax
  % update max count for possible \endthebibliography tack notes
  \@mciteMaxCountUpdate
  % write correct max counter to aux and warn if changed
  \@mciteMaxCountAuxWrite
  % write correct max widths to aux and warn if changed
  \@mciteMaxWidthAuxWrite
  % debug report
  \if@OPTIONmcitedebug
  \typeout{}\relax
  \typeout{** Mciteplus Debug: \string\endmcitethebibliography^^J
  Current Max bibitem count: `\mcitemaxcountbibitem'^^J
  Correct Max bibitem count: `\arabic{mcitebibitemcount}'^^J^^J
  Current Max subitem count: `\mcitemaxcountsubitem'^^J
  Correct Max subitem count: `\@mcitecorrectmaxcountsubitem'^^J^^J
  Current Max bibitem width: `\mcitemaxwidthbibitem'(sp)^^J
  Correct Max bibitem width: `\@mcitecorrectmaxwidthbibitem'(sp)^^J^^J
  Current Max subitem width: `\mcitemaxwidthsubitem'(sp)^^J
  Correct Max subitem width: `\@mcitecorrectmaxwidthsubitem'(sp)}^^J
  \fi}


% warn at end if any \mcitethebibliography requires a rerun due to a max width/count change
\AtEndDocument{\if@mciteLaTeXrerun\@latex@warning@no@line{Rerun to ensure correct mciteplus label max width/count}\fi}

% always ensure \mciteSetMaxWidth{}{}{} and \mciteSetMaxCount{}{}{} are defined in the .aux,
% lest the package be unloaded and the initial .aux still refers to it.
\AtBeginDocument{\if@filesw\immediate\write\@mainaux{\string\providecommand{\string\mciteSetMaxWidth}[3]{\string\relax}}\relax
\immediate\write\@mainaux{\string\providecommand{\string\mciteSetMaxCount}[3]{\string\relax}}\fi}



% hook into system only after all packages have been loaded
\AtBeginDocument{\let\mciteOrgcite\cite\let\mciteOrgnocite\nocite
\if@OPTIONmcitenohooks\else
% hook into system \cite unless user says otherwise
\def\cite{\@mciteCiteWrapper}
\def\nocite{\@mciteNociteWrapper}
\fi}





% special \if macros needed for PKG hooks
% we've got to define these here to shield the \ifcontinuouslabels
% and and \fi from TeX's scanner when multibib is *not* loaded
% as \ifcontinuouslabels will not be defined and TeX would still
% see the \fi when skipping over the code.
%
% multibib 
\def\@mciteMULTIBIBcontinuouslabelsWarn{\relax
\ifmciteResetBibitemCount
   \ifcontinuouslabels
     \typeout{** WARNING: mciteplus is using \string\mciteResetBibitemCounttrue, but multibib was not invoked with `resetlabels' option.}
   \fi
\else
   \ifcontinuouslabels\else
     \typeout{** WARNING: mciteplus is using \string\mciteResetBibitemCountfalse, but multibib was invoked with `resetlabels' option.}
   \fi
\fi}


% bibunits global copy list handler
\def\@mciteBIBUNITSExtraDoListHandler{\ifglobalcitecopy
\mciteDoList{\mciteauxout}{main}{\mciteCiteListArg}\relax
\else
\ifmciteCiteStarFwdArg
\mciteDoList{\mciteauxout}{main}{\mciteCiteListArg}\relax
\fi
\fi}


% natbib command names
\def\@mciteNatbibCiteCmdList{citep,Citep,citet,Citet,citealp,Citealp,citealt,Citealt,citeauthor,Citeauthor,citeyear,citeyearpar,citepalias,citetalias}

% if natbib loaded, save originals at start
\expandafter\ifx\csname ver@natbib.sty\endcsname\relax\else
\AtBeginDocument{\@for\@mcitecurcmdname:=\@mciteNatbibCiteCmdList\do{\relax
\expandafter\let\expandafter\@mcitetmpA\csname \@mcitecurcmdname\endcsname
\expandafter\let\csname mciteOrg\@mcitecurcmdname\endcsname\@mcitetmpA}}
\fi





% *** External Package Hooks ***
\if@OPTIONmcitenohooks\else% hook into packages



% *** natbib.sty hooks
\expandafter\ifx\csname ver@natbib.sty\endcsname\relax\else
\typeout{** mciteplus: Detected natbib.sty. Invoking hooks.}\relax
\AtBeginDocument{\@for\@mcitecurcmdname:=\@mciteNatbibCiteCmdList\do{\relax
% reroute original cite macro \X through \mciteCiteA
% \X -> \mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\mciteOrgX}
\expandafter\@mcitetmptoksA\expandafter=\expandafter{\csname mciteOrg\@mcitecurcmdname\endcsname}\relax
\expandafter\edef\csname \@mcitecurcmdname\endcsname{\noexpand\mciteCiteA{\noexpand\mciteauxout}{\noexpand\mcitetrackID}{\relax}{\relax}{\the\@mcitetmptoksA}}\relax
}}
\fi % if natbib.sty detected




% *** cite.sty hooks
\expandafter\ifx\csname ver@cite.sty\endcsname\relax\else
\typeout{** mciteplus: Detected cite.sty. Invoking hooks.}\relax
\AtBeginDocument{\let\@mciteCITEOrgciten\citen
\def\@mciteCITEciten{\mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\@mciteCITEOrgciten}}\relax
% This will still work even though cite.sty routes \citex through \citen.
% The double calls to mciteplus will be OK as the second call to mciteplus
% will only have a head list of already defined entries and so it will do nothing
% other than write the list to the aux again.
% Not the most elegant approach though.
\def\citen{\@mciteCITEciten}\relax
% Handle the aliases as well.
\def\citenum{\@mciteCITEciten}\relax
\def\citeonline{\@mciteCITEciten}}
\fi % if cite.sty detected



% *** drftcite.sty hooks
\expandafter\ifx\csname ver@drftcite.sty\endcsname\relax\else
\typeout{** mciteplus: Detected drftcite.sty. Invoking hooks.}\relax
\AtBeginDocument{\let\@mciteDRFTCITEOrgciten\citen
\def\@mciteDRFTCITEciten{\mciteCiteA{\mciteauxout}{\mcitetrackID}{\relax}{\relax}{\@mciteDRFTCITEOrgciten}}\relax
% As with cite.sty, this will still work even though drftcite.sty
% routes \citex through \citen.
\def\citen{\@mciteDRFTCITEciten}\relax}
\fi % if drftcite.sty detected



% *** chapterbib hooks
\expandafter\ifx\csname ver@chapterbib.sty\endcsname\relax\else
\typeout{** mciteplus: Detected chapterbib.sty. Invoking hooks.}\relax
% one gotcha is that LaTeX closes and reopens \@partaux so aux handle number
% does not change
\def\mcitetrackID{chapterbib\@currentipfile}
\def\mcitebibtrackID{chapterbib\@currentipfile}
% make a second set of entry status macros for the duplicate bibliographies
% produced under the duplicate option. Won't hurt anything if the duplicate
% bibliography is not used. Note that chapterbib uses the .bbl suffix for
% \@currentipfile when reading the duplicate bibliographies.
\def\mciteExtraDoLists{\mciteDoList{noauxwrite}{chapterbib\@currentipfile.bbl}{\mciteCiteListArg}\relax
% create third set only when chapterbib is using the rootbib option.
% We can't just write this out all the time because the rootbib option can
% cause a conflict in the mciteplus status of a key if that same key is
% used in different parts of the document. And we can't test for the use of
% the chapterbib rootbib option because chapterbib is rerun without the
% rootbib option.
\if@OPTIONmcitechapterbibrootbib
  \mciteDoList{noauxwrite}{chapterbib\jobname}{\mciteCiteListArg}\relax
\fi}
\fi % if chapterbib detected




% *** multibib hooks
\expandafter\ifx\csname ver@multibib.sty\endcsname\relax\else
\typeout{** mciteplus: Detected multibib.sty. Invoking hooks.}\relax
\let\@mciteOrgMULTIBIBnewcites\newcites

% internally braced \nocite with \@aux handler as needed by multibib
% usage: \@mciteMULTIBIBgroupedOrgNocite{multibib section name}{cite list}
\def\@mciteMULTIBIBgroupedOrgNocite#1#2{{\expandafter\let\expandafter\@auxout\csname @auxout#1\endcsname
\mciteOrgnocite{#2}}}

\def\@mciteMULTIBIBnewcites#1#2{\relax
% forward to original \newcites and let it do its thing first
\@mciteOrgMULTIBIBnewcites{#1}{#2}%
% now redo some of what it did our way
\@for\@mciteCurRefName:=#1\do{\relax
%
% build auxout names and track ID
\edef\@mcitetempauxout{\csname @auxout\@mciteCurRefName\endcsname}\relax
\edef\@mcitetemptrackID{multibib\@mciteCurRefName}\relax
%
% reroute original \citeX through \mciteCiteA using \@mciteCurRefName in aux and track
% \citeX -> \mciteCiteA{\@auxoutX}{multibibX}{\relax}
%                      {\let\@citex\mb@@citex\let\@newciteauxhandle\@auxoutX}
%                      {\mciteOrgcite}
% basic command name list
\def\@mciteMULTIBIBCiteCmdList{cite}
% add natbib names if natbib is loaded
\expandafter\ifx\csname ver@natbib.sty\endcsname\relax\else
\edef\@mciteMULTIBIBCiteCmdList{\@mciteMULTIBIBCiteCmdList,\@mciteNatbibCiteCmdList}\relax
\fi
\@for\@mcitecurcmdname:=\@mciteMULTIBIBCiteCmdList\do{\relax
\@mcitetmptoksA=\expandafter{\expandafter{\@mcitetempauxout}}\relax
\expandafter\@mciteAppendToTmpToksA\expandafter{\expandafter{\@mcitetemptrackID}{\relax}}\relax
% install multibib \citeX internals into handler
\edef\@mcitetemp{{\let\noexpand\@citex\noexpand\mb@@citex
\let\noexpand\@newciteauxhandle\csname @auxout\@mciteCurRefName\endcsname}}\relax
\expandafter\@mciteAppendToTmpToksA\expandafter{\@mcitetemp}\relax
% forward to standard \cite (\mciteOrgcite), can't go through current \cite
% as that goes through mcite again and would write entries to standard aux
\expandafter\@mciteAppendToTmpToksA\expandafter{\expandafter{\csname mciteOrg\@mcitecurcmdname\endcsname}}\relax
% define new \citeX wrapper
\expandafter\expandafter\expandafter\def\expandafter\expandafter\csname \@mcitecurcmdname\@mciteCurRefName\endcsname
\expandafter{\expandafter\mciteCiteA\the\@mcitetmptoksA}\relax
}% \do for \@mciteMULTIBIBCiteCmdList
%
% reroute original \nociteX through \mciteCiteA using \@mciteCurRefName in aux and track
% \nociteX -> \mciteCiteA{\@auxoutX}{multibibX}{\relax}
%                      {\relax}
%                      {\@mciteMULTIBIBgroupedOrgNocite}
\@mcitetmptoksA=\expandafter{\expandafter{\@mcitetempauxout}}\relax
\expandafter\@mciteAppendToTmpToksA\expandafter{\expandafter{\@mcitetemptrackID}{\relax}{\relax}}\relax
% forward to standard \@mciteMULTIBIBgroupedOrgNocite, can't go through current \nocite
% as that goes through mcite again and would write entries to standard aux also because
% multibib changes \@auxout, we need to use the internally grouped version with
% the \@aux handler in it
\edef\@mcitetemp{{\noexpand\@mciteMULTIBIBgroupedOrgNocite{\@mciteCurRefName}}}
% define new \nociteX wrapper
\expandafter\@mciteAppendToTmpToksA\expandafter{\@mcitetemp}
\expandafter\expandafter\expandafter\def\expandafter\expandafter\csname nocite\@mciteCurRefName\endcsname
\expandafter{\expandafter\mciteCiteA\the\@mcitetmptoksA}\relax
% now reroute \bibliographyX
% save as \@mciteOrgMULTIBIBbibliographyX
\expandafter\let\expandafter\@mcitetemp\csname bibliography\@mciteCurRefName\endcsname
\expandafter\let\csname @mciteOrgMULTIBIBbibliography\@mciteCurRefName\endcsname\@mcitetemp
\@mcitetmptoksA=\expandafter{\csname @mciteOrgMULTIBIBbibliography\@mciteCurRefName\endcsname}\relax
\expandafter\edef\csname bibliography\@mciteCurRefName\endcsname{\def\@mciteoneshotBIBdecl{\def\noexpand\@mcitecurtrackID{\@mcitetemptrackID}}\the\@mcitetmptoksA}\relax
% we depend on the default \mciteauxout and \mcitetrackID for \cite, \nocite and \mcite
}% end ref name do loop
}% end def \@mcitePKGnewcites
%
% setup multibib BIB hooks
% no need to install bibliography wrapper uaing \@auxoutX as multibbl wrapper alters
% \@auxout to point to \@auxoutX before starting \mcitethebibliography
% Thus, the default bibteckID will work.
% 
% warn if a mismatch between the settings of mciteplus entry label counter resets and those of multibib
\expandafter\@mcitetmptoksA\expandafter=\expandafter{\@mcitepkgBIBdecl}
\addto@hook\@mcitetmptoksA{\@mciteMULTIBIBcontinuouslabelsWarn}
\edef\@mcitepkgBIBdecl{\the\@mcitetmptoksA}
% reroute all \newcites calls through \@mciteMULTIBIBnewcites
\let\newcites\@mciteMULTIBIBnewcites
\fi% if multibib detected



% *** multibbl hooks
\expandafter\ifx\csname ver@multibbl.sty\endcsname\relax\else
\typeout{** mciteplus: Detected multibbl.sty. Invoking hooks.}\relax
% for checking that the user has called \newbibliography before \cite.
\def\@mciteMULTIBBLcheckAuxDefined{\expandafter\ifx\csname\mciteCiteSecIDArg @auxfile\endcsname\relax
\PackageError{mciteplus}{multibbl: Bibliography `\mciteCiteSecIDArg' has not been defined}{Use multibbl's \string\newbibliography\space to
 declare this bibliography before using it in \string\cite.}\relax
\fi}
%\cite -> \mciteCiteB{\secID@auxfile}{multibbl\secID}{create aux track arguments}{\relax}{\mciteOrgcite}}
%\cite -> \mciteCiteB{\secID@auxfile}{multibbl\secID}{create aux track arguments}{\relax}{\mciteOrgcite}}
% we use prehandler to set aux and track arguments to use mciteCiteSecIDArg
\def\@mciteCiteWrapper{\mciteCiteB{Bogus auxout}{Bogus trackID}{\relax
\def\mciteCiteAuxArg{\csname \mciteCiteSecIDArg @auxfile\endcsname}\relax
\def\mciteCiteTrackArg{multibbl\mciteCiteSecIDArg}\@mciteMULTIBBLcheckAuxDefined}{\relax}{\mciteOrgcite}}
% nocite
\def\@mciteNociteWrapper{\mciteCiteB{Bogus auxout}{Bogus trackID}{\relax
\def\mciteCiteAuxArg{\csname \mciteCiteSecIDArg @auxfile\endcsname}\relax
\def\mciteCiteTrackArg{multibbl\mciteCiteSecIDArg}\@mciteMULTIBBLcheckAuxDefined}{\relax}{\mciteOrgnocite}}
% hook into bibliography at start of document, use one shot interface for single use setup of the aux and track ID
\AtBeginDocument{\let\mciteOrgbibliography\bibliography
% we need to update \mcitethebibliography's tracking ID, to reflect what multibbl is using,
% multibbl.sty does not read in non-main aux files. We use the one shot so that the definition is cleared
% after each bibliography (but in this case it would be anyway as it is defined inside the
% \bibliography environment).
\def\bibliography#1#2#3{\def\@mciteoneshotBIBdecl{\relax
  \def\@mcitecurtrackID{multibbl#1}}
  \mciteOrgbibliography{#1}{#2}{#3}}}

\fi% if multibbl detected



% *** bibunits hooks
\expandafter\ifx\csname ver@bibunits.sty\endcsname\relax\else
\typeout{** mciteplus: Detected bibunits.sty. Invoking hooks.}\relax

\def\@mciteBIBUNITSbibunit{\def\mcitetrackID{bibunits\@bibunitname}\relax
\def\mcitebibtrackID{bibunits\@bibunitname}\mciteOrgBIBUNITSbibunit}

\def\@mciteBIBUNITSbu@cite{\@startbibunitorrelax\mciteCiteA{\@bibunitaux}{\mcitetrackID}{\relax}{\@mciteBIBUNITSExtraDoListHandler}{\mciteOrgBIBUNITSbu@cite}}
\def\@mciteBIBUNITSbu@nocite{\@startbibunitorrelax\mciteCiteA{\@bibunitaux}{\mcitetrackID}{\relax}{\@mciteBIBUNITSExtraDoListHandler}{\mciteOrgBIBUNITSbu@nocite}}

\AtBeginDocument{\let\mciteOrgBIBUNITSbu@cite\bu@cite
\let\mciteOrgBIBUNITSbu@nocite\bu@nocite
\let\mciteOrgBIBUNITSbibunit\bibunit
\let\mciteOrgBIBUNITSstd@bibliography\std@bibliography
\let\bibunit\@mciteBIBUNITSbibunit
\let\bu@cite\@mciteBIBUNITSbu@cite
\let\bu@nocite\@mciteBIBUNITSbu@nocite
% have to restore main track ID for global bibliography when using \bibliographyunit
\def\std@bibliography{\def\mcitebibtrackID{main}\mciteOrgBIBUNITSstd@bibliography}}

\fi% if bibunits detected


% *** backref.sty (from hyperref) hooks
\expandafter\ifx\csname ver@backref.sty\endcsname\relax\else
\typeout{** mciteplus: Detected backref.sty. Invoking hooks.}\relax
% disable backref's \bibitem intercept within mcitethebibliography
\expandafter\@mcitetmptoksA\expandafter=\expandafter{\mcitethebibliographyHook}
\addto@hook\@mcitetmptoksA{\def\BR@@lbibitem{\@lbibitem}\def\BR@@bibitem{\@bibitem}}
\edef\mcitethebibliographyHook{\the\@mcitetmptoksA}
%\def\BR@bibitem{\BRorg@bibitem}
% and install our own
\def\mciteBACKREFform{{}\ \BR@backref{\@mcitecurhead}}
\expandafter\@mcitetmptoksA\expandafter=\expandafter{\mciteEndOfBibGroupPresubcloseHook}
\addto@hook\@mcitetmptoksA{\mciteBACKREFform}
\edef\mciteEndOfBibGroupPresubcloseHook{\the\@mcitetmptoksA}
\fi % if backref.sty detected


% *** citeref.sty hooks
\expandafter\ifx\csname ver@citeref.sty\endcsname\relax\else
\typeout{** mciteplus: Detected citeref.sty. Invoking hooks.}\relax
% disable citeref's \bibitem intercepts within mcitethebibliography
\expandafter\@mcitetmptoksA\expandafter=\expandafter{\mcitethebibliographyHook}
\addto@hook\@mcitetmptoksA{\def\@@lbibitem{\@lbibitem}\def\@@bibitem{\@bibitem}}
\edef\mcitethebibliographyHook{\the\@mcitetmptoksA}
%\def\@@lbibitem{\@lbibitem}
%\def\@@bibitem{\@bibitem}
% and install our own
\def\mciteCITEREFform{\bibitempages{\@citerefpages{\@mcitecurhead}}}
\expandafter\@mcitetmptoksA\expandafter=\expandafter{\mciteEndOfBibGroupPresubcloseHook}
\addto@hook\@mcitetmptoksA{\mciteCITEREFform}
\edef\mciteEndOfBibGroupPresubcloseHook{\the\@mcitetmptoksA}
\fi % if citeref.sty detected



% *** detect attempts to use incompatible packages ***
% might be best not to lockout amsrefs and biblatex - maybe somebody wants
% and knows how to use them "in parallel" with mciteplus

% *** incompatible with bibtopic.sty
\expandafter\ifx\csname ver@bibtopic.sty\endcsname\relax\else
\PackageError{mciteplus}{Bibtopic.sty cannot be used with mciteplus.sty}{These two packages won't work together.}\relax
\fi

% *** incompatible with inlinebib.sty
\expandafter\ifx\csname ver@inlinebib.sty\endcsname\relax\else
\PackageError{mciteplus}{inlinebib.sty cannot be used with mciteplus.sty}{These two packages won't work together.}\relax
\fi

% *** incompatible with jurabib.sty
\expandafter\ifx\csname ver@jurabib.sty\endcsname\relax\else
\PackageError{mciteplus}{jurabib.sty cannot be used with mciteplus.sty}{These two packages won't work together.}\relax
\fi

% *** incompatible with opcit.sty
\expandafter\ifx\csname ver@opcit.sty\endcsname\relax\else
\PackageError{mciteplus}{opcit.sty cannot be used with mciteplus.sty}{These two packages won't work together.}\relax
\fi

% *** incompatible with splitbib.sty
\expandafter\ifx\csname ver@splitbib.sty\endcsname\relax\else
\PackageError{mciteplus}{Splitbib.sty cannot be used with mciteplus.sty}{These two packages won't work together.}\relax
\fi
\fi % if hooks enabled


\endinput

